Differential privacy statistical inference for a directed graph network model with covariates

Network data typically contain sensitive relational information, where direct release or sharing may lead to non-negligible privacy violations without proper statistical safeguards. While differential privacy has emerged as a powerful framework for privacy-preserving network data analysis, theoretical understanding remains limited particularly for models incorporating both network structure and nodal attributes. This paper bridges this gap by investigating a directed $\beta$-model with covariates under differential privacy constraints. Our model accounts for both node-level heterogeneity (via $2n$-dimensional degree parameters $\theta$ ) and covariate-driven homogeneity (via a $p$-dimensional parameter $\gamma$). To protect privacy, we introduce a joint Laplace mechanism for releasing network statistics while satisfying differential privacy constraints. Leveraging moment-based estimation techniques, we estimate the parameters of both degree heterogeneity and homogeneity and derive the consistency and asymptotic normality of the differentially private estimators as the network size tends to infinity. Our theoretical findings are validated through numerical simulations and real-world case studies, demonstrating the validity of our theoretical results.

==> Reference.tex <==
\begin{thebibliography}{199}
	
	\bibitem{block2014multidimensional}
	Block P and Grund T,
	Multidimensional homophily in friendship networks, J. Network Science, 2014, 2(2): 189-212.
	
	\bibitem{backstrom2007wherefore}
	Backstrom L, Dwork C, and Kleinberg J,
	Wherefore art thou r3579x? anonymized social networks, hidden patterns, and structural steganography, Proceedings of the 16th international conference on World Wide Web, 2007, 181-190.
	
	\bibitem{dwork2006calibrating}
	Dwork C, McSherry F, Nissim K, et al.,
	Calibrating noise to sensitivity in private data analysis, Theory of Cryptography Conference, 2006, 265-284.
	
	\bibitem{lu2017edge}
	Lu J L, Cai Z P, Wang X M, et al.,
	An edge correlation based differentially private network data release method, J. Security and Communication Networks, 2017.
	
	\bibitem{gao2020protecting}
	Gao T C and Li F, Protecting social network with differential privacy under novel graph model, J. IEEE Access, 2000, 8: 185276--185289.
	
	
	\bibitem{chen2014correlated}
	Chen R, Fung B C M, Yu P S, et al.,
	Correlated network data publication via differential privacy, J. The VLDB Journal, 2014, 23:n653-676.
	
	
	\bibitem{karwa2017sharing}
	Karwa V, Krivitsky P N and Slavkovi{\'c} A B, Sharing social network data: differentially private estimation of exponential family random-graph models, J.Journal of the Royal Statistical Society Series C: Applied Statistics, 2017, 66(3): 481-500.
	
	
	
	\bibitem{salas2023differentially}
	Salas J, Gonz{\'a}lez-Zelaya V, Torra V, et al.,
	David, Differentially Private Graph Publishing Through Noise-Graph Addition, International Conference on Modeling Decisions for Artificial Intelligence, Springer, 2023, 253-264.
	
	
	\bibitem{karwa2016inference}
	Karwa, Vishesh and Slavkovi{\'c},Inference using noisy degrees: Differentially private $\beta$-model and synthetic graphs, J. The Annals of Statistics, 2016, 44(1): 87-112.
	
	\bibitem{yan2021directed}
	Yan T, Directed networks with a differentially private bi-degree sequence, J. Statistica Sinica, 2021, 31(4): 2031-2050.
	
	\bibitem{luo2022jssc}
	Luo J and Qin H, Asymptotic in the Ordered Networks with a Noisy Degree Sequence, J. Journal of Systems Science and Complexity, 2022, 35(3): 1137--1153.
	
	\bibitem{wang2022weighted}
	Wang Q P, Zhang X, Luo J, et al., Weighted directed networks with a differentially private bi-degree sequence, J. Communications in Statistics-Theory and Methods, 2022, 51(2): 285-300.
	
	\bibitem{luo2022affiliation}
	Luo J, Liu T, and Wang Q P, Affiliation weighted networks with a differentially private degree sequence, J. Statistical Papers, 2022, 63(2): 367-395.
	
	
	\bibitem{wang2022two}
	Wang Q P, Yan T, Jiang B Y,et al., Two-mode networks: inference with as many parameters as actors and differential privacy, J. The Journal of Machine Learning Research, 2022, 23(1): 13240--13277.
	
	
	\bibitem{luo2022asymptotic}
	Luo J and Qin H, Asymptotic in a class of network models with a difference private degree sequence, J. Statistics and Its Interface, 2022, 15(3): 383-397.
	
	\bibitem{pan2023differentially}
	Pan L and Hu J W, Differentially private estimation in a class of bipartite graph models, J. Communications in Statistics-Theory and Methods, 2023, 1-20.
	
	\bibitem{yan2023differentially}
	Yan T, Differentially private analysis of networks with covariates via a generalized $beta $-model,J. SCIENCE CHINA Mathematics,10.1007/s11425.
	
	\bibitem{graham2017econometric}
	Graham B S, An econometric model of network formation with degree heterogeneity, J. Econometrica, 2017, 85(4): 1033-1063.
	
	\bibitem{yan2018statistical}
	Yan T, Jiang B Y, Fienberg S E, et al., Statistical Inference in a Directed Network Model withs*, J. Journal of the American Statistical Association, 2019, 114(526): 857-868.
	
	\bibitem{KL1948}
	Kantorovich L V, Functional analysis and applied mathematics, J. Uspekhi Mat Nauk, 1948, 89-185.
	
	
	\bibitem{lazega2001collegial}
	Lazega E, The collegial phenomenon: The social mechanisms of cooperation among peers in a corporate law partnership, Oxford University Press, USA, 2001.
	
	\bibitem{yan2016asymptotics}
	Yan T, Leng C L, and Zhu J, Asymptotics in directed exponential random graph models with an increasing bi-degree sequence, J. The Annals of Statistics, 2016, 44(1): 31-57.
	
	\bibitem{xu2023network}
	Xu M and Wang Q P, A network Poisson model for weighted directed networks with covariates, J. Communications in Statistics-Theory and Methods, 2023, 52(15): 5274--5293.
	
	\bibitem{yamamoto1986error}
	Yamamoto T, Error bounds for Newton's iterates derived from the Kantorovich theorem, J. Numerische Mathematik, 1986, 48(1): 91-98.
	
	
	\bibitem{gragg1974optimal}
	Gragg W B and Tapia R A, Optimal error bounds for the Newton--Kantorovich theorem, J. SIAM Journal on Numerical Analysis, 1974, 11(1): 10-13.
	
	\bibitem{Lang1993}
	Lang S, Real and functional analysis, Springer, New York, 1993.
	
	\bibitem{hoeffding1994probability}
	Hoeffding W, Probability inequalities for sums of bounded random variables, J. The collected works of Wassily Hoeffding, 1994, 409-426.
	
	\bibitem{billingsley1968convergence}
	Billingsley P, Convergence of probability measures, John Wiley \& Sons, Inc, Hoboken, 1968.
	
	
\end{thebibliography}
	
	
	
